One-Loop Partition Functions in Deformed $\mathcal{N}=4$ SYM Theory

We study the thermodynamic behaviour of the real $\beta$- and $\gamma_i$-deformation of $\mathcal{N}=4$ Super Yang-Mills theory on $\mathbb{R}\times S^3$ in the planar limit. These theories were shown to be the most general asymptotically integrable supersymmetric and non-supersymmetric field-theory deformations of $\mathcal{N}=4$ Super Yang-Mills theory, respectively. We calculate the first loop correction to their partition functions using an extension of the dilatation-operator and P\'{o}lya-counting approach. In particular, we account for the one-loop finite-size effects which occur for operators of length one and two. Remarkably, we find that the $\mathcal{O}(\lambda)$ correction to the Hagedorn temperature is independent of the deformation parameters, although the partition function depends on them in a non-trivial way.

==> Macros/MacrosJan.tex <==
%%%%% ABKUERZUNGEN

%%% Math abbreviations

% sets
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\CC}{\ensuremath{\mathbb{C}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\NN}{\ensuremath{\mathbb{N}}}

% groups and algebras
\newcommand{\G}{\ensuremath{G}\xspace}
\newcommand{\UN}{\ensuremath{\text{U}(N)}\xspace}
\newcommand{\SUN}{\ensuremath{\text{SU}(N)}\xspace}
\newcommand{\U}[1]{\ensuremath{\text{U}(#1)}\xspace}
\newcommand{\SU}[1]{\ensuremath{\text{SU}(#1)}\xspace}
\newcommand{\SO}[1]{\ensuremath{\text{SO}(#1)}\xspace}
\newcommand{\GLs}[2]{\ensuremath{\text{GL}(#1|#2)}\xspace}
\newcommand{\SUs}[2]{\ensuremath{\text{SU}(#1|#2)}\xspace}
\newcommand{\PSLs}[2]{\ensuremath{\text{PSL}(#1|#2)}\xspace}
\newcommand{\galgebra}{\ensuremath{\mathfrak{g}}\xspace}
\newcommand{\su}[1]{\ensuremath{\mathfrak{su}(#1)}\xspace}
\newcommand{\so}[1]{\ensuremath{\mathfrak{so}(#1)}\xspace}
\newcommand{\psutctsf}{\ensuremath{\mathfrak{psu}(2,2|4)}\xspace}

%super conformal operators
\newcommand{\superQ}{\mathfrak{Q}}
\newcommand{\superQd}{\dot{\superQ}}
\newcommand{\DilatationD}{D}
\newcommand{\adim}{\gamma}


% Misc
\newcommand{\complexi}{\mathnormal{i}}
\DeclareMathOperator{\idm}{\mathds{1}}
\newcommand{\diag}{\text{diag}}



%%% Math 

% Misc
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\Tr}{\tr}
\DeclareMathOperator{\tr}{tr}
\newcommand{\rtr}[1]{\tr_{#1}}
\newcommand{\colours}{s}
\newcommand{\metric}{\ensuremath{\eta}}
\newcommand{\signature}{\zeta} %{\varsigma}
\newcommand{\cstar}{\ensuremath{\ast}}

% brackets
\newcommand{\ev}[1]{\langle #1 \rangle}
\newcommand{\abs}[1]{|#1|}
\newcommand{\ket}[1]{\mid #1\rangle}
\newcommand{\bra}[1]{\langle#1\mid}
\newcommand{\braket}[2]{\langle#1 \mid #2\rangle}
\newcommand{\comm}[2]{[#1,#2]}
\newcommand{\acomm}[2]{\{#1,#2\}}
\newcommand{\starcomm}[2]{\comm{#1}{#2}_\cstar}
\newcommand{\staracomm}[2]{\acomm{#1}{#2}_\cstar}
\newcommand{\set}[1]{ \{ #1 \} }
%\newcommand{\conditionset}[2]{\set{ #1 \operatorname{|} #2 }}
\newcommand{\state}[1]{\ket{#1}}
\newcommand{\vac}{\operatorname{\mid} 0\operatorname{\rangle}}
%\newcommand{\twositevac}{\state{0\,0}}


% equations
\newcommand{\eqndot}{\, .}
\newcommand{\eqncom}{\, ,}
\newcommand{\nn}{\nonumber}
\newcommand{\nnl}{\nonumber \\}


% Derivatives and integrals
\newcommand{\de}{\operatorname{d}\!}
%\DeclareMathOperator{\dop}{d}
%\newcommand{\measure}[1]{\dop\! #1}
%\newcommand{\Diff}[2]{\frac{\dop^{#2}}{\dop\!{#1}^{#2}}}
%\newcommand{\IntOp}[3]{\int^{#3}_{#2} \!\!\! \dop\! #1 \,}
%\newcommand{\textIntOp}[3]{\int^{#3}_{#2} \! \dop\! #1 \,}
%\newcommand{\MomInt}[2]{\int \frac{\dop^{#2}\!{#1}}{(2\pi)^{#2}}}

%%% References

\newcommand{\appref}[1]{appendix~\ref{#1}}
\newcommand{\Appref}[1]{Appendix~\ref{#1}}
\newcommand{\chapref}[1]{chapter~\ref{#1}}
\newcommand{\Chapref}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{section~\ref{#1}}
\newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\subsecref}[1]{subsection~\ref{#1}}
\newcommand{\tabref}[1]{table~\ref{#1}}
\newcommand{\figref}[1]{figure~\ref{#1}}


%%% Letters

% cal
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% bold
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bq}{\mathbf{q}}

% dotted
\newcommand{\alphadot}{\dot{\alpha}}
\newcommand{\betadot}{\dot{\beta}}
\newcommand{\gammadot}{\dot{\gamma}}
\newcommand{\deltadot}{\dot{\delta}}
\newcommand{\epsilondot}{\dot{\epsilon}}


%%% Text abbreviations
\newcommand{\tHooft}{'t~Hooft\xspace} 
% \renewcommand{\TH}{\ensuremath{T_{\text{H}}}}
\newcommand{\THag}{\ensuremath{T_{\text{H}}}}
%\renewcommand{\H}{{\text{H}}}
\newcommand{\QCD}{{\text{QCD}}}
\newcommand{\stringc}{{\text{s}}}
\newcommand{\AdSCFT}{AdS/CFT\xspace}
\newcommand{\AdSCFTc}{AdS/CFT correspondence\xspace}
\newcommand{\Polya}{P\'{o}lya\xspace}
\newcommand{\Poincare}{Poincar\'{e}\xspace}
\newcommand{\RxSt}{\ensuremath{\mathbb{R}\times S^3}\xspace}
\newcommand{\Nfour}{$\mathcal{N}=4$\xspace}
\newcommand{\NfSYM}{\Nfour SYM\xspace}
\newcommand{\NfSYMt}{\Nfour SYM theory\xspace}
\newcommand{\AdS}[1]{\ensuremath{AdS_{#1}}\xspace}
%\newcommand{\expectationvalue}{expectation value\xspace}
%\newcommand{\expectationvalues}{expectation values\xspace}

% Fields
\newcommand{\ferm}{\psi}
\newcommand{\aferm}{\bar{\psi}}
\newcommand{\scal}{\phi}
\newcommand{\ascal}{\bar{\phi}}
\newcommand{\sufphi}{\varphi}
\newcommand{\cantifstrength}{\bar{\cfstrength}}
\newcommand{\f}{F}
\newcommand{\af}{\bar{\f}}
\newcommand{\gaugefield}{A}
\newcommand{\cder}{D}

% Oscillators
\newcommand{\aosc}{\ba}
\newcommand{\aoscdag}{\aosc^\dagger}
\newcommand{\bosc}{\bb}
\newcommand{\boscdag}{\bosc^\dagger}
\newcommand{\cosc}{\bc}
\newcommand{\coscdag}{\cosc^\dagger}

% occupation numbers
%oscillator kind site type
\newcommand{\oa}[1][ ]{a^{#1}}
\newcommand{\ob}[1][ ]{b^{#1}}
\newcommand{\oc}[1][ ]{c^{#1}}
\newcommand{\od}[1][ ]{d^{#1}}
\newcommand{\oksa}[2][ ]{a^{#1}_{(#2)}}
\newcommand{\oksb}[2][ ]{b^{#1}_{(#2)}}
\newcommand{\oksc}[2][ ]{c^{#1}_{(#2)}}
\newcommand{\oksd}[2][ ]{d^{#1}_{(#2)}}
%\newcommand{\nsite}[1]{n_{(#1)}}

% operators
\newcommand{\centralchargeop}{\ensuremath{\mathcal{C}}}
\newcommand{\centralchargeopdensity}{\ensuremath{C}}
\newcommand{\centralchargeoperatordensity}{\centralchargeopdensity}
\newcommand{\oneloopdop}{\ensuremath{\mathfrak{D}_2}}
\newcommand{\Dzerodensity}{\ensuremath{D_0}}
\newcommand{\Dtwodensity}{\ensuremath{D_2}}
\newcommand{\Dzero}{\ensuremath{\mathfrak{D}_0}}
\newcommand{\Dtwo}{\ensuremath{\mathfrak{D}_2}}


% algebra generators
\newcommand{\Drealalg}{\ensuremath{\mathscr{D}}}
\newcommand{\Prealalg}{\ensuremath{\mathscr{P}}}
\newcommand{\Krealalg}{\ensuremath{\mathscr{K}}}
\newcommand{\Lrealalg}{\ensuremath{\mathscr{L}}}
\newcommand{\Jrealalg}{\ensuremath{\mathscr{J}}}


% Operators
\newcommand{\Dalg}{\ensuremath{\mathfrak{D}}}
\newcommand{\Halg}{\ensuremath{\mathfrak{H}}}


% Colour
\DeclareMathOperator{\T}{T}
%\newcommand{\onetrace}[1]{\tr\T^{#1}}
%\newcommand{\twotrace}[2]{\tr\T^{#1}\T^{#2}}
%\newcommand{\threetrace}[3]{\tr\T^{#1}\T^{#2}\T^{#3}}
%\newcommand{\fourtrace}[4]{\tr\T^{#1}\T^{#2}\T^{#3}\T^{#4}}
%\newcommand{\threetracecomm}[3]{\tr\T^{#1}\comm{\T^{#2}}{\T^{#3}}}

% Coupling tensors

%\newcommand{\Qtilde}[4]{\tilde{Q}_{#4 #3}^{#1 #2}}
%\newcommand{\Qbare}[4]{Q_{ #4 #3}^{#1 #2}}
%\newcommand{\Qhat}[4]{\hat{Q}_{#4 #3}^{#1 #2}}
%
%\newcommand{\Qt}[4]{\Qtilde{#1}{#2}{#3}{#4}}
%\newcommand{\Qonehalf}[4]{\Qbare{#1}{#2}{#3}{#4}}
%\newcommand{\Q}[4]{\Qhat{#1}{#2}{#3}{#4}}
%
%\newcommand{\ro}[3]{({\rho}_{#1})_{#2 #3}}
%\newcommand{\rodag}[3]{(\rho^{\dagger #1})^{#2 #3}}
%\newcommand{\rotil}[3]{(\tilde{\rho}_{#1})^{#2 #3}}
%\newcommand{\rotildag}[3]{(\tilde{\rho}^{\dagger #1})_{#2 #3}}


% Christoph stuff
%\newlength{\eqoff}

% SUSY stuff
%\DeclareMathOperator{\D}{D}
%\DeclareMathOperator{\barD}{\vphantom{\D}\smash[t]{\bar{\mathrm{D}}}}



% Misc

\newcommand{\indups}[1]{_{\mathrm{\scriptscriptstyle #1}}}
\newcommand{\gym}{g\indups{YM}}
\newcommand{\YM}{{\mathrm{\scriptscriptstyle YM}}}
%  
% \newcommand{\g}[1]{{\gamma_{#1}}}
% \newcommand{\cg}[1]{{\cos{\gamma_{#1}}}}
%\DeclareMathOperator{\premax}[1]{max}
\newcommand{\maxset}[1]{\max{\{#1\}}}
\newcommand{\minset}[1]{\min{\{#1\}}}
\newcommand{\singleE}[2]{\operatorname{E}_{#1,#2}}
\newcommand{\E}[4]{\operatorname{E}_{#1,#2}\otimes\operatorname{E}_{#3,#4}}
%\newcommand{\func}[2][red]{\textcolor{#1}{f(#2)}}
\newcommand{\deltafct}[1]{\delta(#1)}

\DeclareMathOperator{\phaneq}{\phantom{{}=}}
\newcommand{\phaneqtimes}{\qquad \times}
\newcommand{\dzeroev}{{D_0}}
\newcommand{\colors}{s}
\newcommand{\colorshat}{\hat{s}}
\newcommand{\e}{\operatorname{e}}
\newcommand{\numberdot}[1]{#1}







% Derivatives and integrals
\DeclareMathOperator{\dop}{d}
\newcommand{\measure}[1]{\dop\! #1}
\newcommand{\Diff}[2]{\frac{\dop^{#2}}{\dop\!{#1}^{#2}}}
\newcommand{\IntOp}[3]{\int^{#3}_{#2} \!\!\! \dop\! #1 \,}
\newcommand{\textIntOp}[3]{\int^{#3}_{#2} \! \dop\! #1 \,}
\newcommand{\MomInt}[2]{\int \frac{\dop^{#2}\!{#1}}{(2\pi)^{#2}}}



%%% Letters








% occupation numbers
\newcommand{\akind}[1][ ]{a^{#1}}
\newcommand{\bkind}[1][ ]{b^{#1}}
\newcommand{\ckind}[1][ ]{c^{#1}}
\newcommand{\dkind}[1][ ]{d^{#1}}
\newcommand{\akindsite}[2][ ]{a^{#1}_{(#2)}}
\newcommand{\bkindsite}[2][ ]{b^{#1}_{(#2)}}
\newcommand{\ckindsite}[2][ ]{c^{#1}_{(#2)}}
\newcommand{\dkindsite}[2][ ]{d^{#1}_{(#2)}}
\newcommand{\nsite}[1]{n_{(#1)}}










% SUSY stuff
\DeclareMathOperator{\D}{D}
\DeclareMathOperator{\barD}{\vphantom{\D}\smash[t]{\bar{\mathrm{D}}}}



